Towards Controllable Natural Language Inference through Lexical Inference Types

Explainable natural language inference aims to provide a mechanism to produce explanatory (abductive) inference chains which ground claims to their supporting premises. A recent corpus called EntailmentBank strives to advance this task by explaining the answer to a question using an entailment tree \cite{dalvi2021explaining}. They employ the T5 model to directly generate the tree, which can explain how the answer is inferred. However, it lacks the ability to explain and control the generation of intermediate steps, which is crucial for the multi-hop inference process. % One recent corpus, EntailmentBank, aims to push this task forward by explaining an answer to a question according to an entailment tree \cite{dalvi2021explaining}. They employ T5 to generate the tree directly, which can explain how the answer is inferred but cannot explain how the intermediate is generated, which is essential to the multi-hop inference process. In this work, we focus on proposing a controlled natural language inference architecture for multi-premise explanatory inference. To improve control and enable explanatory analysis over the generation, we define lexical inference types based on Abstract Meaning Representation (AMR) graph and modify the architecture of T5 to learn a latent sentence representation (T5 bottleneck) conditioned on said type information. We also deliver a dataset of approximately 5000 annotated explanatory inference steps, with well-grounded lexical-symbolic operations. Experimental results indicate that the inference typing induced at the T5 bottleneck can help T5 to generate a conclusion under explicit control.

==> sections/future_work.tex <==
\section{Future Work} \label{sec:future}

==> sections/limitation.tex <==
% \section{Limitations} \label{sec:limit}
% Evaluation metrics: as described in Table \ref{tab:metrics_with_inference_type} the metrics, such as BLEURT, cannot accurately reflect the correctness of generated conclusion. Therefore, how to quantitatively evaluate the correctness of predicted conclusions from the inference side should be considered in the future.
    
% \noindent \textbf{2.} Sentence representation: inference types can help T5 to generate an expected conclusion, which has been proved in this work. However, can it help sentence bottleneck T5 is under-explored. From the experiment, we can observe that the information of inference type as Encoder input is lost because of the bottleneck of the sentence representation. Therefore, how can inference type better inject into the sentence bottleneck T5 should be explored in the future.

==> tables/arg1_exp.tex <==

\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{6}{c}{ARG1: disentanglement metrics (forward: $T$)} \\ \hline

classifier & train & accuracy & precision & recall  & f1 score \\ \hline
\multirow{3}{*}{KNN} & O & 0.958 & 0.958 & 0.958  & 0.958 \\
 & U & 0.951 & 0.951 & 0.951  & 0.951 \\
 & C & \textbf{0.969} & \textbf{0.969} & \textbf{0.969}  & \textbf{0.969}  \\ \hline
 
\multirow{3}{*}{NB} & O & 0.907 & 0.907 & 0.907  & 0.907 \\
 & U & 0.926 & 0.926 & 0.926  & 0.926 \\
 & C & \textbf{0.956} & \textbf{0.956} & \textbf{0.956}  & \textbf{0.956} \\ \hline
 
\multirow{3}{*}{SVM} & O & 0.956 & 0.956 & 0.956  & 0.956 \\
& U & 0.953 & 0.953 & 0.953 & 0.953 \\
 & C & \textbf{0.958} & \textbf{0.958} & \textbf{0.958}  & \textbf{0.958} \\ \toprule
\end{tabular}
}

\caption{disentanglement of ARG1 between Optimus (O), unsupervised INN (U), and supervised INN (S) (KNN: k-neighbours, NB: naive bayes, SVM: support vector machine).} \label{tab:arg1_exp}
\end{table}
\end{center}

==> tables/baselines.tex <==
% \begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{2.5pt}
% \resizebox{7.8cm}{!}{
\small
\centering
\renewcommand\arraystretch{1.1}
\begin{tabular}{cp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
% \multicolumn{5}{}{pred conclusion \textit{vs} golden conclusion} \\ \hline
Baseline & Injection & BLEU & Cosine & BLEURT & Loss $\downarrow$ & PPL $\downarrow$ \\ \hline
% \multirow{3}{*}{\shortstack{T5 \\ small}} & DE & 0.46 & 0.96 & 0.23 & 0.49 & 1.33 \\ 
% & DP & 0.53 & 0.96 & 0.25 & 0.51 & 1.38 \\ 
% & \cellcolor{lightgray}EP & \cellcolor{lightgray}\textbf{0.61} & \cellcolor{lightgray}\textbf{0.97} & \cellcolor{lightgray}\textbf{0.39} & \cellcolor{lightgray}\textbf{0.45} & \cellcolor{lightgray}\textbf{1.22} \\ \hline
% & NO & 0.58 & 0.96 & 0.35 & 0.61 & 1.65 \\ \toprule
\multicolumn{7}{c}{\textit{Encoder-Decoder models without bottleneck}}  \\ \hline
\multirow{4}{*}{\shortstack{T5 original \\ (small)}} & DE & \underline{0.55} & \underline{0.96} & \underline{0.30} & 0.53 & 1.44 \\ 
& DP & 0.59 & 0.96 & 0.34 & 0.58 & 1.57 \\ 
& EP & \cellcolor{lightgray}\textbf{0.65} & \cellcolor{lightgray}\textbf{0.97} & \cellcolor{lightgray}\textbf{0.45} & \cellcolor{lightgray}\textbf{0.52} & \cellcolor{lightgray}\textbf{1.41} \\
& NO & 0.54 & 0.96 & 0.22 & \underline{0.69} & \underline{2.22} \\ \hline
% & NO & 0.61 & 0.96 & 0.38 & \underline{0.82} & \underline{2.22} \\ \hline

\multirow{4}{*}{\shortstack{T5 original \\ (base)}} & DE & \underline{0.46} & \underline{0.96} & \underline{0.23} & 0.49 & 1.33 \\ 
& DP & 0.53 & 0.96 & 0.25 & 0.51 & 1.38 \\ 
& EP & \cellcolor{lightgray}\textbf{0.61} & \cellcolor{lightgray}\textbf{0.97} & \cellcolor{lightgray}\textbf{0.39} & \cellcolor{lightgray}\textbf{0.45} & \cellcolor{lightgray}\textbf{1.22} \\ 
& NO & 0.57 & 0.96 & 0.33 & \underline{0.61} & \underline{1.65} \\ \hline
% & NO & 0.58 & 0.96 & 0.35 & \underline{0.61} & \underline{1.65} \\ \hline

\multirow{4}{*}{\shortstack{Bart (base)}} & DE & 0.44 & 0.94 & 0.03 & 0.55 & 1.49 \\ 
& DP & \underline{0.38} & \underline{0.93} & \underline{-0.42} & \textbf{0.48} & \textbf{1.30} \\ 
& EP & \cellcolor{lightgray}\textbf{0.57} & \cellcolor{lightgray}\textbf{0.96} & \cellcolor{lightgray}\textbf{0.23} & 0.58 & 1.57 \\ 
& NO & 0.54 & 0.96 & 0.17 & \underline{0.63} & \underline{1.71} \\ \hline \hline
\multicolumn{7}{c}{\textit{Encoder-Decoder models with bottleneck}}  \\ \hline
\multirow{4}{*}{\shortstack{T5 bottleneck \\ (base, 768)}} & DE & 0.41 & 0.92 & -0.07 & 0.67 & 1.82 \\ 
& DP & 0.41 & 0.92 & -0.05 & \textbf{0.67} & \textbf{1.82} \\ 
& EP & \underline{0.33} & \underline{0.90} & \underline{-0.22} & 1.17 & 3.18 \\ 
& NO & \cellcolor{lightgray}\textbf{0.46} & \cellcolor{lightgray}\textbf{0.93} & \cellcolor{lightgray}\textbf{0.01} & \underline{1.26} & \underline{6.49} \\ \hline
\multirow{4}{*}{\shortstack{Optimus \\ (BERT-GPT2, 768)}} & DE & 0.26 & 0.79 & -1.11 & 0.87 &  \\ 
& DP & 0.25 & 0.80& -1.14& 0.85 &  \\ 
& EP & 0.09 & 0.74 & -1.17 & 1.11 & \\
& NO & 0.07 & 0.74 & -1.20 & 1.10 & \\ \hline 
\multirow{4}{*}{\shortstack{LSTM DAE \\ \cite{10.1145/1390156.1390294}}} & DE &  &  &  & &  \\ 
& DP & & & & &  \\ 
& EP & & & & & \\
& NO & & & & & \\ \hline \hline
\multicolumn{7}{c}{\textit{Auto-regressive models}}  \\ \hline
\multirow{3}{*}{\shortstack{LlaMA(7B)}} & DE &  &  &  & &  \\ 
& DP & & & & &  \\ 
& NO & & & & & \\ \toprule

% \multirow{4}{*}{\shortstack{FlanT5 \\ (small)}} & DE & 0.35 & \textbf{0.90} & \textbf{-1.06} & \textbf{0.72} & \textbf{1.95} \\ 
% & DP & \textbf{0.36} & 0.89 & -1.13 & 0.74 & 2.01 \\ 
% & EP & 0.24 & 0.89 & -1.29 & 0.87 & 2.36 \\ 
% & NO & \underline{0.22} & \underline{0.89} & \underline{-1.33} & \underline{0.99} & \underline{2.69} \\ \toprule

% \multirow{3}{*}{\shortstack{Bart \\ base}} & DE & 0.41 & 0.92 & -0.07 & 0.67 & 1.82 \\ 
% & DP & 0.41 & 0.92 & -0.05 & 0.67 & 1.82 \\ 
% & EP & \underline{0.33} & \underline{0.90} & \underline{-0.22} & 1.17 & 3.18 \\ \hline
% & NO & 0.46 & 0.93 & 0.01 & \underline{1.26} & \underline{6.49} \\ \toprule

% \multirow{4}{*}{\shortstack{GPT2}} & DE &  &  &  & &  \\ 
% & DP & & & & &  \\ 
% & EP & & & & & \\
% & NO & & & & & \\ \toprule

\end{tabular}
% }
\caption{Quantitative evaluation of test cases (best and worst results are highlighted in bold and underlined, respectively). Specification for abbreviation. INJ: ways for injecting the information of inference types into the model, it includes DE: decoder end, DP: decoder prefix, EP: encoder prefix, NO: no inference type. PPL is perplexity, Loss is cross entropy.} \label{tab:metrics_with_inference_type}
\end{table}
% \end{center}

==> tables/failure_generation.tex <==
\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, title=Inference type prediction]
\underline{P1: meters m are a metric / si unit used for} \\ \underline{measuring length} \\
\underline{P2: a classroom is usually measured in meter} \\ 

GOLD: meter is the si unit that can be used to measure a classroom \\
GOLD Type: ARG-INS \\
PRED: a classroom is usually measured in \textcolor{blue}{a si unit for measuring length} \\
PRED Type: FRAME-SUB
\end{tcolorbox}
\caption{Example of wrong inference type predicted by the original T5(base). More examples are provided in Table \ref{tab:more_example_2}.}
\label{tab:failure_example}
\end{table}

==> tables/latent_arithmetic.tex <==
\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, title=Linear latent arithmetic]

\end{tcolorbox}

\caption{Linear latent arithmetic.}
\label{tab:latent_arithmetic}
\end{table}

==> tables/llm_label_prediction.tex <==
\begin{table}[ht!]
\centering
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
\begin{tabular}{ccc}
\toprule
Baseline & Num & Accuracy \\ \hline
\shortstack{CoT-T5 (11b)\cite{kim2023cot}} & 0 &  \\ 
\shortstack{Flan-T5 (xl)} & 0 &  \\
\shortstack{Flan-T5 (xxl)} & 0 & \\
\shortstack{GPT-3.5-turbo-0125}& 0 & \\
\shortstack{GPT-4-0613} & 0 & \\
\shortstack{llama3-8b-8192} & 0 &  \\
\shortstack{llama3-70b-8192} & 0 & \\ \toprule
\end{tabular}
}
\caption{Inference type label prediction via In-context learning (ICL).} \label{tab:predict_llm}
\end{table}

==> tables/metrics_new.tex <==
\begin{table}[ht!]
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
\renewcommand\arraystretch{1}
\begin{tabular}{ccccc}
\toprule
Baseline & INJ & BLEU & Cosine & BLEURT \\ \hline
\multicolumn{5}{c}{\textit{Transformer: baselines without bottleneck}}  \\ \hline
\multirow{4}{*}{\shortstack{T5 \\ original \\ (small)}} & DE & \underline{0.55} & \underline{0.96} & \underline{0.30} \\ 
& DP & 0.59 & 0.96 & 0.34 \\ 
& EP & \textcolor{blue}{\textbf{0.65}} & \textcolor{blue}{\textbf{0.97}} & \textcolor{blue}{\textbf{0.45}}\\
& NO & 0.54 & 0.96 & 0.22 \\ \hline

\multirow{4}{*}{\shortstack{T5 \\ original \\ (base)}} & DE & \underline{0.46} & \underline{0.96} & \underline{0.23} \\ 
& DP & 0.53 & 0.96 & 0.25  \\ 
& EP & \textcolor{blue}{\textbf{0.61}} & \textcolor{blue}{\textbf{0.97}} & \textcolor{blue}{\textbf{0.39}} \\ 
& NO & 0.57 & 0.96 & 0.33 \\ \hline
\multirow{4}{*}{\shortstack{Bart \\ (base)}} & DE & 0.44 & 0.94 & 0.03 \\ 
& DP & \underline{0.38} & \underline{0.93} & \underline{-0.42} \\ 
& EP & \textcolor{blue}{\textbf{0.57}} & \textcolor{blue}{\textbf{0.96}} & \textcolor{blue}{\textbf{0.23}} \\ 
& NO & 0.54 & 0.96 & 0.17 \\ \hline 
\multirow{4}{*}{\shortstack{T5 \\ original \\ (large)}} & DE & 0.60 & 0.97 & 0.46 \\ 
& DP & 0.64 & 0.97 & 0.44 \\ 
& EP & \textcolor{blue}{\textbf{0.67}} & \textcolor{blue}{\textbf{0.97}} & \textcolor{blue}{\textbf{0.50}}\\ 
& NO & 0.57 & 0.96 & 0.31 \\ \hline
\multirow{4}{*}{\shortstack{Flan-T5 \\ (large)}} & DE & 0.01 & 0.73 & -1.34 \\ 
& DP & 0.01 & 0.73 & -1.34 \\ 
& EP & \textcolor{blue}{\textbf{0.21}} & \textcolor{blue}{\textbf{0.87}} & \textcolor{blue}{\textbf{-1.04}} \\ 
& NO & 0.20 & 0.87 & -1.14 \\ \hline
\multirow{4}{*}{\shortstack{T5 \\ original \\ (3b, enc)}} & DE &  \\ 
& DP & \\ 
& EP & 0.70 & 0.97 & 0.57 \\ 
& NO & 0.68 & 0.97 & 0.55 \\ \hline
\multirow{4}{*}{\shortstack{CoT-T5 \\ \cite{kim2023cot} \\(11b, zero-shot)}} & & \\ 
& EP & \textcolor{blue}{\textbf{0.50}} & \textcolor{blue}{\textbf{0.97}} & \textcolor{blue}{\textbf{0.36}}\\ 
& NO & 0.46 & 0.96 & 0.31\\
& \\ \hline \hline
\multicolumn{5}{c}{\textit{CasualLM: baselines without bottleneck}}  \\ \hline

\multirow{3}{*}{\shortstack{GPT2 \\ (large)}} & DE & 0.02 & 0.87 & -1.15  \\ 
& DP & \textcolor{blue}{\textbf{0.08}} & \textcolor{blue}{\textbf{0.90}} & \textcolor{blue}{\textbf{-0.91}} \\ 
& NO & 0.07 & 0.90 & -0.93 \\ \hline 
\multirow{3}{*}{\shortstack{GPT2 \\ (xl)}} & DE &  \\ 
& DP & \\ 
& NO & \\ \hline
\multirow{2}{*}{\shortstack{LlaMA \\ (7b, zero-shot)}}
& DP &\\ 
& NO &\\ \hline 
\multirow{2}{*}{\shortstack{LlaMA \\ (13b, zero-shot)}}
& DP & \\ 
& NO & \\ \hline \hline
\multicolumn{5}{c}{\textit{sentence baselines with bottleneck}}  \\ \hline
\multirow{4}{*}{\shortstack{T5 \\ bottleneck \\ (base)}} & DE & 0.35 & 0.91 & -0.15 \\ 
& DP & 0.39 & 0.91 & -0.13 \\ 
& EP & \textcolor{blue}{\textbf{0.42}} & \textcolor{blue}{\textbf{0.92}} & \textcolor{blue}{\textbf{-0.07}} \\
& NO & \underline{0.35} & \underline{0.91} & \underline{-0.20} \\ \hline
\multirow{4}{*}{\shortstack{Optimus \\ (BERT-GPT2)}} & DE & \textcolor{blue}{\textbf{0.26}} & \textcolor{blue}{\textbf{0.80}} & \textcolor{blue}{\textbf{-1.11}} \\ 
& DP & 0.25 & 0.79 & -1.14 \\ 
& EP & 0.09 & 0.74 & -1.17 \\
& NO & \underline{0.07} & \underline{0.74} & \underline{-1.20} \\
\toprule
\end{tabular}
}
\caption{Quantitative evaluation of test cases (best and worst results are highlighted in \textbf{\textcolor{blue}{bold}} and \underline{underlined}, respectively). Specification for abbreviation. INJ: ways for injecting the information of inference types into the model, it includes DE: decoder end, DP: decoder prefix, EP: encoder prefix, NO: no inference type.} \label{tab:metrics_with_inference_type}
\end{table}

==> tables/more_examples_2.tex <==
\begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{3pt}
\small
\centering
\resizebox{15cm}{!}{
% \renewcommand\arraystretch{1.4}
\begin{tabular}{p{4.5cm}p{4.5cm}p{4.5cm}p{1.5cm}}
\toprule
Premises & Sentence bottleneck T5 & Golden conclusion & BLEURT \\ \hline
P1: feeling is when an living thing senses through touch & soft feelings is when an animal senses soft sensations through touch & soft is a kind of feeling & -0.52 \\ 
P2: soft is a kind of touch sensation &&& \\ \hline

% P1: photosynthesis is a kind of process in which plants convert carbon dioxide and water and solar energy into carbohydrates and food and oxygen for themselves & a plant is a source of oxygen through photosynthesis & plants are a source of carbohydrates through photosynthesis & -0.08 \\

P2: if a plant uses a process to convert something into something else then that plant is a source of that something else through that process &&& \\ \hline 

P1: burning coal emits sulfur dioxide & burning coal and burning oil are two sulfur dioxide emitters & burning coal and oil emit sulfur dioxide & -0.15 \\
P2: burning oil emits sulfur dioxide &&& \\ \hline

% P1: limestone is a kind of sedimentary rock that is formed by deposition / cementation and marble is a kind of metamorphic rock that is formed by rocks being exposed to extreme heat and pressure & limestone form a kind of sedimentary rock that is formed by deposition / cementation and marble is a kind of metamorphic rock that is formed by rocks being exposed to extreme heat & limestone and marble are different classes of rock and are formed by different methods & -0.58 \\
% P2: class is a property of a rock and includes values of sedimentary / metamorphic / igneous &&& \\ \hline

P1: a leaf is a part of a green plant & chlorophyll is a part of green plants & a leaf is a part of a green plant that contains chlorophyll & -0.15 \\
P2: leaves contain chlorophyll &&& \\ \hline

P1: some bacteria are good for humans by helping digestion & an example of good digestion is stomach acid breaking down food & some bacteria are good for humans by helping to break down food & -0.34 \\
P2: digestion is when stomach acid breaks down food &&& \\ \hline

P1: producing thrust causes an animal to move & a squid producing thrust causes an animal to move & a squid produces thrust by pushing water out of its body & -0.07 \\
P2: a squid produces a stream of water out of its body that causes it to move \\ \hline

P1: the iron nail has rusted & rusting is when iron reacts chemically with water and oxygen & a chemical reaction has happened on the iron nail & -0.95 \\ 
P2: rusting is when iron chemically reacts with water and oxygen &&& \\ \hline

P1: metal is an electrical conductor & metal is an electrical conductor and metal is a thermal conductor & metal can conduct electricity and heat & -0.12\\
P2: metal is a thermal conductor &&& \\ \hline

P1: a needle is a part of a pine tree & a pine tree has a needle part and a leaf part & a needle is a kind of leaf that is a part of a pine tree & -0.15 \\
P2: a needle is a kind of leaf &&& \\ \hline

P1: helium is a kind of element & helium and pure substances are both elements & helium is a pure substance & -0.10 \\
P2: elements are pure substances &&& \\ \toprule
\end{tabular}
}
\caption{T5 bottleneck: more examples with low BLEURT scores.} \label{tab:more_example_1.1}
\end{table}
\end{center}

==> tables/more_examples_3_1.tex <==
% \begin{center}
\begin{table}[ht!]
\scriptsize
% \setlength\tabcolsep{3pt}
% \small
\centering
\resizebox{15cm}{!}{
% \renewcommand\arraystretch{1.4}
\begin{tabular}{p{6cm}p{3cm}p{6cm}}
\toprule
Premises & Inference Type & T5 bottleneck  \\ \hline
P1: a pumpkin contains seeds & ARG-INS & fruit is part of a pumpkin that contains seeds  \\ 
P2: fruit contains seeds & FRAME-CONJ & a fruit contains seeds \\ 
 & FRAME-SUB & a pumpkin is a kind of plant \\ \hline
P1: sunlight is a kind of solar energy & ARG-INS & water is a kind of resource that is used by plants for growth \\
P2: water and sunlight are resources for plants & FRAME-CONJ & plants and water are resources that require water and energy \\ 
& ARG-SUB & plants use water and sunlight to produce energy \\ \hline
P1: to move something can mean to transfer something & ARG-SUB & flowing can mean to transfer energy \\
P2: flowing is a kind of movement for energy & INF & if something flows, then that energy will flow \\
& FRAME-CONJ & moving can transfer energy and mean flowing \\
& ARG-INS & flowing can be a kind of transfer of something \\ 
& ARG/PRED-GEN & transferring energy with flowing can be seen as transferring energy \\ \hline
P1: if a pot is exposed to a stove then that pot may become hot & COND-FRAME & the pot may become hot \\ 
P2: the pot is exposed to a stove & ARG/PRED-GEN & the pot may be a source of heat \\ \hline
P1: eating something has a negative impact on that something & FRAME-SUB & eating cacti has a negative impact on that cacti \\
P2: some animals eat cacti & PRED-SUB & animals have a negative impact on cacti \\
& ARG-INS & some animals have a negative impact on cacti by eating cacti \\ \hline

P1: seeing requires light & ARG-SUB & reading requires light \\
P2: reading requires seeing & FRAME-CONJ & reading and feeling can both be used \\
& INF & if something is visible then that something will be seen \\ \toprule
\end{tabular}
}
\caption{T5 bottleneck: controllable NLI via inference type.} \label{tab:more_example_3.1}
\end{table}
% \end{center}

==> tables/more_examples_4.tex <==
\begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{3pt}
\small
\centering
\resizebox{15cm}{!}{
% \renewcommand\arraystretch{1.4}
\begin{tabular}{p{4cm}p{4cm}p{3cm}p{2cm}p{2cm}}
\toprule
Premises & Predicted conclusion & Golden conclusion & PRED type & GOLD type \\ \hline
P1: webbed feet have a positive impact on an aquatic animal's survival & webbed feet have a positive impact on an aquatic animal's adaptation & webbed feet are a kind of adaptation for aquatic animals & FRAME-SUB & ARG/PRED-GEN \\ 
P2: an adaptation has a positive impact on an animal's survival &&&& \\ \hline

P1: burning something is a kind of action & burning something requires burning something & if something occurs by burning something else, then burning that something else is required for that something to occur & COND-FRAME & FRAME-SUB \\
P2: if something occurs by performing an action, then that action is required for that something to occur &&&& \\ \hline

P1: food contains nutrients & a protein is a kind of food that contains a protein & food contains proteins & ARG-INS & ARG-SUB \\
P2: a protein is a kind of nutrient &&&& \\ \hline

P1: the environment has changed from a body of water to mountains & the atmosphere is found on the surface of earth & the environments on the crustal surface of earth have changed from a body of water to mountains & FRAME-SUB & ARG-INS \\ 
P2: environments are found on the crustal surface of earth &&&& \\ \hline

P1: ocean water is made of hydrogen and oxygen & ocean water is becoming more common on earth & oxygen is the most common element found in the compounds that make up ocean water & FRAME-SUB & ARG-INS \\
P2: oxygen is more common than hydrogen on earth &&&& \\ \hline

P1: bees have a positive impact on plant reproduction & help of bees has a positive impact on plant reproduction & bees help plant reproduction & ARG-SUB & PRED-SUB \\
P2: helping something has a positive impact on that something &&&& \\ \toprule
\end{tabular}
}
\caption{Original T5: inference type prediction.} \label{tab:more_example_2}
\end{table}
\end{center}

==> tables/more_examples_without_if.tex <==
\begin{center}
\begin{table}[ht!]
\scriptsize
\setlength\tabcolsep{3pt}
\small
\centering
\resizebox{15cm}{!}{
% \renewcommand\arraystretch{1.4}
\begin{tabular}{p{4cm}p{4cm}p{3.5cm}p{3.5cm}}
\toprule
Premises & Original T5 & Sentence bottleneck T5 & Golden conclusion \\ \hline
P1: a human is a kind of object & a child is a kind of object & a child is a kind of object & a child is a kind of object \\ 
P2: a child is a kind of young human &&& \\ \hline

P1: a plant / living thing requires nutrients to grow & food is an essential ingredient for a plant to grow & food is a kind of fertilizer that can be used by plants & a plant requires food to grow \\ 
P2: food contains nutrients for living things &&& \\ \hline

P1: bees have a positive impact on plant reproduction & helping bees has a positive impact on plant reproduction & helping bees has a positive impact on plant reproduction & bees help plant reproduction \\
P2: helping something has a positive impact on that something &&& \\ \hline

P1: a doorbell is a kind of electric device & closing an electric circuit causes a doorbell to function & closing of a doorbell causes the doorbell to function & an electric circuit causes a doorbell to function \\ 
P2: closing an electric circuit causes an electrical device to function \\ \hline

P1: an animal gets the energy it needs to run from food & an animal gets the energy it needs to run from food & a dog gets the energy it needs to run from food & a dog gets the energy it needs to run from food \\
P2: a dog is a kind of animal \\ \hline

% P1: as the number of fish in a lake increases the number of insects in that lake will decrease & as the number of fish in a lake increases, the number of insects in that lake will decrease & as the number of fish in a lake increases, the number of insects in that lake will decrease & if the number of fish in a lake increases there will be fewer insects in that lake \\
% P2: if something decreases in number then there will be fewer of that something &&& \\ \hline

P1: if something is made of minerals then that something contains minerals & rock contains minerals & a rock is a kind of rock & a rock contains minerals \\
P2: rock is made of minerals &&& \\ \hline

P1: ocean water is made of hydrogen and oxygen & ocean water is more common on earth than on earth & ocean water is more common than oxygen on earth & oxygen is the most common element found in the compounds that make up ocean water \\ 
P2: oxygen is more common than hydrogen on earth &&& \\ \hline

P1: water will change from a liquid to a solid by decreasing heat energy &  water will change from a liquid to a solid by decreasing temperature & water will change from a liquid to a solid by decreasing temperature & water will change from a liquid to a solid by decreasing the temperature \\
P2: temperature is a measure of heat energy &&& \\ \hline

% P1: if something is required to perform a process then that something can be absorbed to perform that process & if something is required to do photosynthesis then that something can be absorbed to do photosynthesis & if something is required to perform photosynthesis then that something can be absorbed to perform photosynthesis & if something is required to perform photosynthesis then that something can be absorbed to perform photosynthesis \\
% P2: photosynthesis is a kind of process &&& \\ \hline

P1: volvox is a kind of protist & volvox is a protist & volvox is a kind of protist that reproduces sexually & volvox is a kind of protist that reproduces sexually \\
P2: volvox reproduces sexually &&& \\ \hline

% P1: sound requires matter to travel & sound can travel within a vacuum & sound can travel through a vacuum & sound cannot travel through a vacuum \\
% P2: a vacuum has no matter in it &&& \\ \hline
\end{tabular}
}
\caption{More examples for original T5 and sentence bottleneck T5.} \label{tab:more_example_1}
\end{table}
\end{center}
